Limiting the Spread of Fake News on Social Media Platforms by Evaluating Users' Trustworthiness

Today's social media platforms enable to spread both authentic and fake news very quickly. Some approaches have been proposed to automatically detect such "fake" news based on their content, but it is difficult to agree on universal criteria of authenticity (which can be bypassed by adversaries once known). Besides, it is obviously impossible to have each news item checked by a human. In this paper, we a mechanism to limit the spread of fake news which is not based on content. It can be implemented as a plugin on a social media platform. The principle is as follows: a team of fact-checkers reviews a small number of news items (the most popular ones), which enables to have an estimation of each user's inclination to share fake news items. Then, using a Bayesian approach, we estimate the trustworthiness of future news items, and treat accordingly those of them that pass a certain "untrustworthiness" threshold. We then evaluate the effectiveness and overhead of this technique on a large Twitter graph. We show that having a few thousands users exposed to one given news item enables to reach a very precise estimation of its reliability. We thus identify more than 99% of fake news items with no false positives. The performance impact is very small: the induced overhead on the 90th percentile latency is less than 3%, and less than 8% on the throughput of user operations.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigconf-xelatex.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-sigconf-xelatex.pdf:  sample-sigconf-xelatex.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	xelatex $<
	- bibtex $*
	xelatex $<
	xelatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do xelatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigconf-xelatex.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes
		

==> sections/evaluation-old.tex <==
\section{Evaluation}
\label{sec:evaluation}

%% We evaluate the effectiveness of our system under parameters that we believe correspond the closest to a real-world deployment.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/tweet-popularity}
\caption{Popularity distribution of the $1024$ most popular items in our sample dataset, peaking at over 750k shares.}
\label{fig:tweet-popularity}
%\vspace{-.3cm}
\end{figure}

We perform our evaluation of \systemname\ using a real-world Twitter graph of over 41M users \cite{Kwak10www}.
To get a realistic distribution of item popularity, we rely on a set of tweets obtained by crawling Twitter.
Out of over 35M tweets, the popularity (retweet count) of the 1024 most popular tweets is depicted in \cref{fig:tweet-popularity}.
In what follows:

\begin{enumerate}
\item We explore \systemname' capacity of detecting fake news.
\item We measure the performance penalty of our prototype implementation when plugged into Twissandra \cite{twissandra},
  a Cassandra-based Twitter clone.
\end{enumerate}

We show that \systemname\ can effectively detect fake news items with high accuracy,
even using a small number of fact-checked news items.
$1024$ items are sufficient to prevent the display of a fake item in over 99\% of the cases, while never preventing a true news item from being displayed.
In a simulated propagation of $500$ viral fake news items, \systemname\ reduces the number of times such an item is viewed from $588$ million to $101$ thousand. On average, this corresponds to a fake item being shown to $200$ users instead of one million.
The impact on system performance is small for both throughput (a decrease of $9$\% on average) and latency (average increase by $1$\%).

\subsection{\systemname' Fake News Detection Capability}
\label{sec:effectiveness-of-detection}

This section presents \systemname' capability of detecting fake news, demonstrated through simulation.
We first describe our simulation methodology, followed by the obtained results.

\subsubsection{\textbf{Simulation Methodology}}\ \\
\label{sec:simulation-methodology}

We evaluate \systemname' fake news detection capability by simulating the propagation of news items over the social graph.
Our simulation proceeds in two steps:
\begin{enumerate}
\item \emph{UCR creation}: determining the UCR (i.e., $v_T, s_T, v_F, s_F$) for each user based on propagation of fact-checked news items.
\item \emph{Fake item detection}: using the UCRs obtained in the previous step, we measure how effectively fake news items can be detected using \systemname.
\end{enumerate}
Note that in a real system these two steps happen continuously and concurrently.
We first discuss three important parameters of our simulation
and then proceed to describing in detail the two simulation steps mentioned above.

\begin{table}
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{name} & \textbf{description} & \textbf{example} \\
\hline
\simparam{r} & Number of fact-checked items & 1024 \\
\hline
\simparam{f} & Fraction of fake fact-checked items & $1/4$ \\
\hline
\simparam{msp} & Maximum probability of & $1/64$ \\
 & a user sharing an item & \\
\hline
\end{tabular}
\vspace{.3cm}
\caption{Important parameters of \systemname}
\vspace{-.3cm}
\label{tab:params}
\end{table}

\paragraph{\textbf{Simulation Parameters}}

Three important parameters (summarized in \cref{tab:params}) influence \systemname' behavior.
%% We experimented with many different parametrizations and we present our system's behavior for parameter combinations that we find realistic and representative.
%% As we explain in detail later, the higher any of these parameters, the better \systemname\ performs.

\begin{itemize}
\item \textbf{\simparam{r}} is the number of fact-checked news items that we use during UCR creation.

\item \textbf{\simparam{f}} represents the fraction of fake items among the fact-checked ones.
Note that in reality we do not have complete control over this parameter (the outcome of fact-checking is not known a-priori).
However, we can pick items for fact-checking based on how likely they are to be fake
(e.g., based on some content-based machine learning algorithm, or on the commonly known reputation / credibility of their sources).
We use the value $\simparam{f} = 1/4$ for most of our simulations, but also show the impact of varying \simparam{f} on the created UCRs.

\item \textbf{\simparam{msp}} (\underline{m}ax \underline{s}hare \underline{p}robablility) models users' intrinsic sharing behavior: how likely users are to share news items they are exposed to.
For each simulated user $u$, we set $P_T(u)$ and $P_F(u)$ (see \cref{sec:detection-theory}) to a value chosen uniformly at random between $0$ and \simparam{msp}.
Note that \simparam{msp} is \emph{not} a system parameter of \systemname.
It models how users (which are external to \systemname) react to news items.
We do not know what \simparam{msp} is in reality.
We even expect it to be different for different news items, as, in reality, some items become viral (modeled by a high \simparam{msp}) and some do not (modeled by a low \simparam{msp}).
However, as we show later, regardless of what the real value of \simparam{msp} is,
\systemname\ effectively prevents fake items from going viral.
\end{itemize}

%% To present \systemname\ for a big and small value of \simparam{f}, we pick the $1/4$ and $1/64$, respectively.
%% Note that \simparam{f} refers to the fraction of fake items among the \emph{fact-checked} ones, and in general we can control which items are fact-checked and which are not.
%% If we try to pick popular items for fact-checking that are likely to be fake (e.g., based on some content-based machine learning algorithm, or items originating at sources known for spreading fake content), we can achieve a high fraction of fake items among those that we fact-check, making even \simparam{f} $=1/4$ a realistic value.

%% For \simparam{msp}, we pick $1/16$ and $1/64$\footnote{The expected probability of a user sharing an item is $\frac{\simparam{msp}}{2}$. (\cref{sec:simulation-setup})} as the respective big and small values.
%% Since we are concerned mostly about viral items, we choose the values for \simparam{msp} accordingly.
%% In our experiments we observe that \simparam{msp} $=1/16$ is the smallest value for which news items naturally become viral.
%% By ``viral'' we mean that an item naturally propagates to orders of magnitude more users than it was initially introduced to.
%%  %% for which the number of users exposed to it is orders of magnitude bigger than the number of users the item has been initially introduced to.
%% For \simparam{msp} $=1/32$ already, those numbers of users are of the same order of magnitude.
%% In order to illustrate how \systemname\ behaves for even smaller values, we also present experiments using \simparam{msp} $=1/64$.

%% COMMENT (M): mps depends on the tweet itself in reality, which is NOT
%% modeled by our system. However, tweets with low msp don't spread
%% naturally, and tweets with a high msp are efficiently handled by
%% \systemname.




%% Since we consider a limited subset of the tweets, our sample might not include some popular tweets.
%% This puts our estimation on the conservative side, as using more popular items would only improve the performance of our system.

%% We model the behavior of each user $u$ by $P_T(u)$ and $P_F(u)$, the respective probabilities that the user shares a true and a fake news item when exposed to it.
%% For each user, we initialize these share probabilities to random values uniformly distributed between 0 and \simparam{msp} (for maximal share probability).


\paragraph{\textbf{UCR Creation}}

To create UCRs, we propagate \simparam{r} items through the social graph.
We assign each of the \simparam{r} items a target share count.
The target share count corresponds to the number of retweets of a tweet in our dataset,
starting at the most popular one. % and using each tweet only once.
We randomly assign a (ground) truth value to each propagated item based on \simparam{f},
i.e., each item is fake with probability \simparam{f}.

The propagation itself proceeds by exposing a random user $u$ to the propagated item $X$ and having $u$ decide (probabilistically, based on $P_T(u)$ and $P_F(u)$) whether to share $X$ or not.
If $u$ shares $X$, we show $X$ to all $u$'s followers that have not yet seen it.
We repeat this process until one of the following conditions is fulfilled.
\begin{enumerate}
\item The target number of shares is reached.
  In this case we abort propagation immediately, possibly leaving some users without the possibility to decide whether to share $X$ or not.
\item At least 80\% of users have been exposed to $X$, at which point we consider the network saturated.
  This applies especially for small \simparam{msp} values, where the network becomes saturated without reaching the target share count.
  %% Such aborts have a negative impact on our results, since a fact-checked item affects fewer UCRs than it would in reality on a bigger social graph.
  %% In this sense, our simulations are thus a conservative approximation of the expected real-world behavior.
\end{enumerate}

%% An interesting detail about item propagation is the order in which we expose users to items.
%% For each item, we maintain a set of users that should be exposed to that item.
%% Whenever a user decides to share an item, we add all her followers to this set.
%% Users from this set are then exposed to the item in random order.
%% This is crucial, as with a more naive deterministic approach such as DFS traversal of the user graph, users would be exposed to items unevenly.
%% Especially for higher values of \simparam{msp} and lower target share counts, users appearing at the beginning of other users' lists of followers would be more likely to be exposed to an item than users at the end of the follower lists.
%% This would result in some users being exposed to many items (and thus have good UCRs) at the expense of other users.
%% Exposing items to users in random order solves this issue.

During item propagation, we keep track of how many true/fake items each user has seen/shared and update the UCRs accordingly.
%% Assuming all those items have been fact-checked, we update the UCRs accordingly.
%% We measure how various system parameters influence the quality of the obtained UCRs.
%% In particular,
%% \begin{enumerate}
%% \item How many fact-checked items users were exposed to,
%% \item How many UCRs have a relevant score, and
%% \item What are the values of these scores
%% \end{enumerate}



\paragraph{\textbf{Fake Item Detection}}

%% After having created the UCRs by simulating the propagation of fact-checked news items, we measure how effectively the obtained UCRs can be used to detect fake news.
In order to measure \systemname' fake news item detection capability,
we propagate $1000$ items through the social graph ($500$ fake and $500$ true).
We inject each item once, by making a random user $u$ share it.
The propagation happens as in the previous phase, with two important differences:
\begin{itemize}
\item We consider the item not fact-checked, and thus do not update $u$'s UCR.
  Instead, whenever $u$ is exposed to an item, we update that item's rating using the $u$'s UCR score.
  We use the share score if $u$ also shares the item, otherwise we use the view score (see \cref{sec:computing-fake-probability}).
\item We only propagate each item once, without re-inserting it when propagation dies off naturally.
\end{itemize}
When the probability of an item being fake reaches $p_0 = 0.999999$, we save the number of users exposed to it so far.
We continue spreading the item until the propagation stops naturally, to obtain the number of views that would occur in the absence of \systemname.

%% We consult $u$'s profile and include its view contribution (if $u$ did not share the item) or share contribution (if $u$ shared the item) in the computation of the item rating.
%% We measure:
%% \begin{enumerate}
%% \item The number of users that need to be exposed to an item before being reasonably certain that the item is fake.
%% This certainty is represented by the probability threshold $p_0 = 0.999999$.
%% If an item's probability of being fake exceeds $p_0$, we consider that item fake.
%% \item Total number of users exposed to the item.
%% \item Number of users exposed to the item if its propagation stops after being detected as fake.
%% \item Number of users that are prevented from being exposed to true items, if their propagation stops after being wrongly identified as fake.
%% \end{enumerate}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/reviewed-numContribsAbs}
\caption{The number of relevant UCR scores increases with both \simparam{r}, the number of fact-checked news items, and \simparam{f}, the fraction of these items that is fake.}
\label{fig:fact-checked-numContribsAbs}
%\vspace{-.3cm}
\end{figure}

\subsubsection{\textbf{Simulation Results}}\ \\

We now experimentally demonstrate \systemname' capability to effectively detect fake news items.
First we briefly describe how fact checking affects UCR creation and we discuss the choice of the used simulation parameters.
We then present our main result, namely the end-to-end impact of \systemname\ on the number of times users are exposed to fake news.

\paragraph{\textbf{Effectiveness of Fact-checkers}}

\systemname\ relies on fact-checked items to create UCRs.
Since a few most popular items usually reach a large number of users (see \cref{fig:tweet-popularity}),
our intuition is that checking only relatively few news items can result in obtaining sufficiently many useful UCRs.

While several aspects of UCRs influence \systemname' behavior,
due to space limitations we restrict ourselves to one representative metric of the overall quality of the UCRs present in the system:
the total number of UCRs with a useful UCR score.
We consider a UCR score useful if it is different from $1$,
i.e. when it makes a contribution to the rating of an item exposed to the corresponding user.

For this experiment, we choose $\simparam{msp} = 1/16$,
because (as we noticed empirically) this is a value where many items start naturally going viral.
By ``viral'' we mean that an item naturally propagates to orders of magnitude more users than it was initially introduced to.
%% For $\simparam{msp} = 1/32$ already, those numbers of users are of the same order of magnitude.

\Cref{fig:fact-checked-numContribsAbs} depicts how the number of relevant UCRs depends on \simparam{r},
the number of fact-checked items.
We see that fact-checking as few as 1024 news items has an impact on over 13M UCR scores,
which is one third of the whole user population.

The impact of \simparam{f} (the fraction of fake news items among the fact-checked ones) on UCRs is also shown in \cref{fig:fact-checked-numContribsAbs}.
While still assuming the majority of items being true, the higher the \simparam{f} parameter, the more useful UCRs we obtain.
This effect is due to the requirement of balanced UCRs described in \cref{sec:design}.

For the rest of our simulations, we use $\simparam{r} = 1024$ and $\simparam{f} = 1/4$,
as they provide good UCRs while still being a conservative choice.
FactCheck.org, for example, is one of many fact-checking initiatives that exist world-wide \cite{politifact,snopes,wpfactchecker,truthorfiction,fullfact}.
It checked several hundreds of popular stories only during the year 2017, the majority of which turned out to be false or misleading.

\paragraph{\textbf{Fake News Detection Capability}}
\label{sec:overall-effect}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/msp-viewCnt}
\caption{Fake news spreading with \systemname, as a function of \simparam{msp}. For low \simparam{msp}, news items do not become viral. For high \simparam{msp}, \systemname\ blocks the vast majority of fake news items.}
\label{fig:msp-viewCnt}

%\vspace{-.3cm}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/credulix-detail.pdf}
\caption{Fake news spreading with \systemname, as a function of \simparam{msp}, for different social graph sizes.}
\label{fig:msp-relative}
\end{figure}

The ultimate goal of \systemname\ is preventing fake news items from becoming viral on social media.
%% while allowing true news items to spread freely.
To this end, we measure the number of times a user is exposed to a fake news item in two scenarios:
%% We thus start by showing the overall effect of \systemname\ on fake news propagation.
%% To visualize this effect, we consider two scenarios:
\begin{enumerate}
\item Vanilla (natural) propagation of fake news items.
\item Propagation of fake items, where we stop propagating an item when \systemname\ labels it as fake.
\end{enumerate}
\Cref{fig:msp-viewCnt} presents results for items with varying rates of ``virality'', modeled by our \simparam{msp} simulation parameter.
It shows how many times a user has been exposed to a fake item, cumulatively over the $500$ fake items that we disseminate.
We can see that regardless of how viral the items would naturally become,
\systemname\ is able to timely detect the fake items before they spread to too many users.
\systemname\ restricts the number of views (cumulative over $500$ items) from hundreds of millions to tens or hundreds of thousands.%
\footnote{Analogously to a vaccine, \systemname\ needs \emph{some} fake news in order to function well,
as some users being exposed to fake news are crucial for obtaining meaningful UCRs.
Preventing the spreading of the vast majority of fake news might temporarily impair the effectiveness of \systemname, leading to an increased number of users being exposed to fake news.
This, in turn, reinforces \systemname' fake news detection capability.
We leave the study of such dynamic behavior to future work,
but we expect the fake news blocking rate to stabilize.
}

Especially nowadays, considering the increasing responsibility being attributed to social network providers as mediators of information,
it is crucial that true news items are not accidentally marked as fake.
We thus consider it very important to avoid false positives, i.e. true items being incorrectly labeled as fake.
None of these experiments encountered even a single false positive.

To have a closer look at the fake news detection rate,
we plot the percentage of fake items displayed with \systemname\ in \cref{fig:msp-relative}.
The more viral the items get (i.e. the higher the \simparam{msp} value), the more effective \systemname\ becomes at fake item detection.
Intuitively, the more items users share, the more precisely we are able to estimate their sharing behavior.

While not visible in the plot, it is worth noting that not only the relative amount of viewed fake items decreases, but also the \emph{absolute} one.
(One could think that the relative decrease for \systemname\ is only due to an absolute increase for Baseline.)
Interestingly, with increasing tendency of items to go viral (i.e. increasing \simparam{msp}),
even the \emph{absolute} number of displayed fake items decreases.
This effect is due to a higher \simparam{msp} value ensuring more spreading of (both true and fake) news items in our UCR creation phase (see \cref{sec:simulation-methodology}).
This in turn produces better UCRs, increasing \systemname' effectiveness.

\Cref{fig:msp-relative} also conveys the effect of the size of the social graph on the performance of \systemname.
On a smaller graph of 1M users generated with the SNAP generator \cite{snapnets},
\systemname\ achieves a lower fake item detection rate.
This is because the impact of fact-checked items is smaller on a small graph, leading to fewer users with relevant UCR scores.
%% , on which the effectiveness of \systemname\ relies.
This result suggests that on a real social graph, which is even larger than the one we use, \systemname\ would perform even better than in our simulation.

%% As we will explain in detail later, the parameter most influential to \systemname' behavior is \simparam{msp}.
%% The higher \simparam{msp}, the more quickly and accurately we are able to detect fake news items.

%% We show that even so, regardless of \simparam{msp}, fake news items never become viral when \systemname\ is in place.
%% \cref{fig:msp-viewCnt} depicts how the number of users exposed to a fake item depends on \simparam{msp}, for both above-mentioned scenarios.
%% The "Vanilla" lines coincide, because without \systemname, fake item propagation does not depend on \simparam{r} or \simparam{f}.
%% Note that for low values of \simparam{msp}, an item naturally does not spread enough to become viral.
%% As \simparam{msp} grows, our system becomes more and more effective at detecting fake news items, preventing them from spreading at an early stage of propagation.

%% We do not include plots for true news items as those also coincide with the top 3 "Vanilla" lines in both scenarios (both with and without \systemname).
%% This means that the \systemname 's impact on true news items is negligible.


% \cref{fig:msp-viewCnt} contains 6 lines, 3 of which coincide.
% The 3 coinciding lines at the top represent the the number of times a fake item is shown to a user, without the use of \systemname\ (Vanilla)
% The 3 lines at the bottom represent the number of times a fake item is shown to a user with \systemname, for 3 different parametrizations.
% It is clear that from the image that \systemname\ is able to prevent the propagation of fake items, while leaving true items to propagate freely.

%% In the rest of \cref{sec:effectiveness-of-detection}, we present other interesting measurements that help explain the behavior of \systemname.

% So far we studied the effectiveness of our solutions to sub-problems of fake news elimination.
% We now present the end-to-end effect of our system on the spreading of fake news items through a social network.
% We are interested in how many users are actually exposed to fake news as compared to the number of users who would have been affected if our system was not in place.

% As becomes evident from the previously mentioned results, the most crucial parameter determining the effectiveness of our system is \simparam{msp}.
% In reality, the probability of an item being shared by a user is not static, but depends also on the item itself, which is not captured by our simulations.
% This is what, in reality, makes the difference between a viral news item and one that does not become viral.

% The crucial role of the $msp$ parameter lies in ensuring good user profiles, as can be seen in Figure ??.
% This is natural, as a higher $msp$ during the propagation of fact-checked news items ensures a higher number of users being exposed to these items.
% This not only helps increase the user profile scores more, but, most crucially, increases the chance that a profile with high score will also have a strong contribution.

% In our simulations, we use the same static value for $msp$ throughout both profile creation and fake item detection.
% From this point of view, Figure ?? is a conservative approximation of reality, as it is the most viral items that are being fact-checked, corresponding to a rather high $msp$ value.

%% First, we study the effect of fact-checking popular news items on UCRs.
%% Since a few most popular items usually reach a large number of users (see \cref{fig:tweet-popularity}), our intuition is that checking only relatively few news items can create ``good'' UCRs.
%% % that are sufficiently good for effective fake news detection.
%% The general quality of a UCR could be expressed in terms of the number of fact-checked items that user has been exposed to.
%% However, due to the way we compute UCRs in practice (see \cref{sec:design-principles}), the number of fact-checked items relevant for a UCR is only $\min(v_T, v_F)$.
%% \cref{fig:fact-checked-score} shows the average value of $\min(v_T, v_F)$ over all users as a function of \simparam{r}, i.e., the number of fact-checked items.

% \begin{figure}
% \centering
% \includegraphics[width=\columnwidth]{figures/reviewed-score}
% \caption{Average value of $\min(v_T, v_F)$ over all users, as a function of \simparam{r}, \simparam{f}, and \simparam{msp}. It increases with \simparam{r} and \simparam{f}, but is unaffected by \simparam{msp}.}
% \label{fig:fact-checked-score}
% %\vspace{-.3cm}
% \end{figure}

%% Note that the values increase not only with the number of fact-checked items, but also with \simparam{f}, the overall fraction of fake news in the system.
%% This is due to the fact that having a more even distribution of true and fake fact-checked news items, $\min(v_T, v_F)$ increases while $(v_T + v_F)$ remains the same.
%% While the value of $\min(v_T, v_F)$ gives us an insight about the relevance of $r$ and $f$, maximizing it is necessary, but not sufficient for efficient fake news detection.
%% A user $U$ might be exposed to many true and fake fact-checked items, but if $U$ does not share any of these items, $U$'s UCR score is still $1$ and thus not useful for fake news detection.
%% The same goes for a user sharing all items she is exposed to.

%% The most important property of a UCR is its score (see \cref{sec:design-principles}).
%% Recall that an item rating is computed as a product of UCR scores for all users exposed to that item.
%% Thus, the more UCRs have a score different from 1, the more effectively fake news items can be detected.

%% \cref{fig:fact-checked-numContribsAbs} shows the number of UCR scores different from $1$, depending on the number of fact-checked items \simparam{r}.
%% This time, the results depend not only on \simparam{f}, but on \simparam{msp} as well.
%% For the reasons explained above, the more likely a user is to share an item, the more likely it is that her UCR will have a relevant score.

% \begin{figure}
% \centering
% \includegraphics[width=\columnwidth]{figures/reviewed-contribFact}
% \caption{The UCR score values also increase with all of \simparam{r}, \simparam{f}, and \simparam{msp}.}
% \label{fig:fact-checked-contribFact}
% %\vspace{-.3cm}
% \end{figure}

%% \begin{figure}
%% \centering
%% \includegraphics[width=\columnwidth]{figures/viewCnt-detectionRate}
%% \caption{Effectiveness of fake news item detection for \simparam{r}~$=1024$. We display the CDF of fake news items detected, depending the number of users exposed to each item. The horizontal axis uses a logarithmic scale.}
%% \label{fig:viewCnt-detectionRate}
%% %\vspace{-.3cm}
%% \end{figure}

%% It is not only important how many UCRs with relevant scores there are, but what values these scores have.
%% A score close to $1$ is not as useful as a score with a bigger difference to $1$.
%% The further the UCR scores are from $1$, the fewer of them need to be considered to reach the same level of confidence in an item being true or fake.
%% In \cref{fig:fact-checked-contribFact}, we plot the average factor by which a UCR score differs from $1$.
%% As expected, the bigger \simparam{msp}, \simparam{f} and \simparam{r}, the better the score.

%% \subsubsection{Fake News Detection}

%% %% Previously we only studied how various parameters affect the quality of user profiles.
%% In this experiment, we show how effectively \systemname\ detects fake news items.
%% We are interested in the number of views necessary for fake item detection.
%% I.e., how many users have to be exposed to a fake news item in order for the system to detect it as fake.
%% Assuming that the system would block the propagation of a news item detected to be fake, this metric directly expresses how effectively \systemname\ can be used to prevent exposing users to fake news.

%% \cref{fig:viewCnt-detectionRate} plots the fractions of detected fake items relative to the number of users that have been exposed to those items.
%% We see that for \simparam{f} $=1/4$ and \simparam{msp} $=1/16$, all fake items are detected after being viewed by $8196$ users, while most fake items -- 93.6\% and 99.8\% -- are already revealed after being seen by $2048$ and $4096$ users respectively.
%% For the small \simparam{msp} $=1/64$, it might take tens of thousands of user views until an item is detected as fake.
%% However, in the presented experiments, the propagation of these items often died off naturally even before sufficient number of UCRs could be considered (see also \cref{sec:overall-effect}).
%% None of the items reached $2^{17} \approx 130$k users.


%% The point on the trade-off between false positives and false negatives can be tuned using the threshold that needs to be exceeded by a item's probability of being fake in order for the item to be considered fake.
%% We tend to choose a number very close to 1 for this threshold in order to avoid false positives.
%% For 3 out of the 4 experiments in \cref{fig:viewCnt-detectionRate}, we did not observe any false positives.
%% In the experiment with the most pessimistic parametrization of \simparam{f} $=1/64$ and \simparam{msp} $=1/64$, the rate of false positives was less than $1.8\%$.


\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/latency-experiments-figure.pdf}
\caption{Throughput and latency cost of \systemname.}
\vspace{-.3cm}
\label{fig:system-eval-fig}
\end{figure*}

\subsection{\systemname\ Overhead}
In this section we evaluate \systemname' impact on user operation (viewing and sharing) throughput and latency when plugged into a social network.

\subsubsection{\textbf{Experimental Setup}}\ \\

Here we evaluate an implementation of \systemname\ as a stand-alone Java plugin.
We implement a Twitter clone\footnote{Where the share and view operations are identical to \cref{fig:tweet-operation,fig:timeline-operation}}.
From this point forward, we refer to our Twitter clone as the \emph{Baseline}
and to the system with \systemname\ plugged in as \systemname.
For the data store of the Baseline we use Twissandra's data store\cite{twissandra},
running Cassandra version 2.2.9\cite{cassandra}.

We conduct our evaluation on a 48-core machine,
with four 12-core Intel Xeon E7-4830 v3 processors operating at 2.1 GHz,
512 GB of RAM and a 400 GB SSD Samsung 843T, running Ubuntu 16.04.
We run our experiments on a real-world Twitter graph of over 41M users \cite{Kwak10www}, as in \cref{sec:effectiveness-of-detection}.
Each experiment consists of 16 worker threads concurrently performing operations on the social network (sharing items or viewing news feeds).
Each operation is chosen at random, according to the given workload probability distribution.
Each user is chosen uniformly at random from the all the users in the social network graph.

We run two types of workloads.
The first has 90\% view operations and 10\% share operations (already a high percentage of share operations for a realistic social network). The second is a view-only workload. We run each experiment 5 times and we take the average of the results. For the sake of fairness, in each experiment, both \systemname\ and the Baseline use the same execution trace, which was generated a priori. An execution trace is a list of user IDs and operations (e.g., user1:share, user2:view etc.). For all our experiments we consider a user to be influential if they are among the 5\% most followed users.

\subsubsection{\textbf{Experimental Results}}\ \\

\Cref{fig:system-eval-fig} conveys the latencies of user operations, along with the throughput of \systemname\ relative to the Baseline.
The mixed workload is shown on the left side, and the view-only workload is shown on the right side of the figure.

The additional overhead in terms of throughput and latency incurred by \systemname\ is low.
The throughput penalty caused by \systemname\ is between 3\% (in the view-only workload) and 9\% (in the mixed workload).
The impact on throughput is predominantly caused by \systemname' background tasks, as detailed in \cref{sec:design}. 

Latency increases by at most 3\%, at the $90^{th}$ percentile.
The low overhead in latency is due to \systemname\ keeping its computation  outside the critical path.
Standard deviation of latencies is high both for the Baseline and for \systemname, for both post and check operations.
The high variation in latency is caused by the intrinsic differences between the users;
for instance, post operations of a user with more followers need to propagate to more users than posts of users with few or no followers.

The high $99^{th}$ percentile latency for both systems results from Twissandra (our Baseline) being implemented in Java,
a language that is (in)famous for its garbage collection breaks.
Certain operations, during which garbage collection is performed by the JVM, thus experience very high latencies.
This effect is not inherent to the system itself,
but is merely an artifact of its Java implementation and can be avoided by using a language with explicit memory management.
The impact of garbage collection is stronger with \systemname\ than with Baseline,
as \systemname\ creates more short-lived objects in memory to orchestrate its background tasks.
In addition to the intrinsic differences between users discussed above,
garbage collection also significantly contributes to the high standard deviation observed in all latencies.

%% For identical traces run by the Baseline and by \systemname, the latency standard deviation is higher in \systemname.
%% This is due to the fact that, while a significant fraction of the posts are not tracked (thus incurring no overhead),
%% for the posts that are tracked, \systemname\ does perform additional operations.
%% Even if the bulk of the work is performed in the background,
%% there is still overhead associated to starting the background task,
%% causing an increase in latency. 

%% We also notice a significant difference in the 99th percentile latency (18\% in the mixed workload and 40\% in the view-only workload) between \systemname\ and the Baseline.
%% This is due to the fact that \systemname\ is generating background-task objects in order to track items on the read path.
%% These tasks are small and short lived, thus adding extra work for the garbage collector compared to the Baseline.
%% Note that this limitation of the implementation can be avoided in a language providing manual memory management,
%% for example by using a pre-allocated memory pool for such tasks and recycling the memory. 


==> sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

%% We evaluate the effectiveness of our system under parameters that we believe correspond the closest to a real-world deployment.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/tweet-popularity}
\caption{Popularity distribution of the $1024$ most popular items in our sample dataset, peaking at over 750k shares.}
\label{fig:tweet-popularity}
%\vspace{-.3cm}
\end{figure}

We perform our evaluation of \systemname\ using a real-world Twitter graph of over 41M users \cite{Kwak10www}.
To get a realistic distribution of item popularity, we rely on a set of tweets obtained by crawling Twitter.
Out of over 35M tweets, the popularity (retweet count) of the 1024 most popular tweets is depicted in \cref{fig:tweet-popularity}.
In what follows:

\begin{enumerate}
\item We explore \systemname' capacity of detecting fake news.
\item We measure the performance penalty of our prototype implementation when plugged into Twissandra \cite{twissandra},
  a Cassandra-based Twitter clone.
\end{enumerate}

We show that \systemname\ can effectively detect fake news items with high accuracy,
even using a small number of fact-checked news items.
$1024$ items are sufficient to prevent the display of a fake item in over 99\% of the cases, while never preventing a true news item from being displayed.
In a simulated propagation of $500$ viral fake news items, \systemname\ reduces the number of times such an item is viewed from $588$ million to $101$ thousand. On average, this corresponds to a fake item being shown to $200$ users instead of one million.
The impact on system performance is small for both throughput (a decrease of $9$\% on average) and latency (average increase by $1$\%).

\subsection{\systemname' Fake News Detection Capability}
\label{sec:effectiveness-of-detection}

This section presents \systemname' capability of detecting fake news, demonstrated through simulation.
We first describe our simulation methodology, followed by the obtained results.

\subsubsection{\textbf{Simulation Methodology}}\ \\
\label{sec:simulation-methodology}

We evaluate \systemname' fake news detection capability by simulating the propagation of news items over the social graph.
Our simulation proceeds in two steps:
\begin{enumerate}
\item \emph{UCR creation}: determining the UCR (i.e., $v_T, s_T, v_F, s_F$) for each user based on propagation of fact-checked news items.
\item \emph{Fake item detection}: using the UCRs obtained in the previous step, we measure how effectively fake news items can be detected using \systemname.
\end{enumerate}
Note that in a real system these two steps happen continuously and concurrently.
We first discuss three important parameters of our simulation
and then proceed to describing in detail the two simulation steps mentioned above.

\begin{table}
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{name} & \textbf{description} & \textbf{example} \\
\hline
\simparam{r} & Number of fact-checked items & 1024 \\
\hline
\simparam{f} & Fraction of fake fact-checked items & $1/4$ \\
\hline
\simparam{msp} & Maximum probability of & $1/64$ \\
 & a user sharing an item & \\
\hline
\end{tabular}
\vspace{.3cm}
\caption{Important parameters of \systemname}
\vspace{-.3cm}
\label{tab:params}
\end{table}

\paragraph{\textbf{Simulation Parameters}}

Three important parameters (summarized in \cref{tab:params}) influence \systemname' behavior.
%% We experimented with many different parametrizations and we present our system's behavior for parameter combinations that we find realistic and representative.
%% As we explain in detail later, the higher any of these parameters, the better \systemname\ performs.

\begin{itemize}
\item \textbf{\simparam{r}} is the number of fact-checked news items that we use during UCR creation.

\item \textbf{\simparam{f}} represents the fraction of fake items among the fact-checked ones.
Note that in reality we do not have complete control over this parameter (the outcome of fact-checking is not known a-priori).
However, we can pick items for fact-checking based on how likely they are to be fake
(e.g., based on some content-based machine learning algorithm, or on the commonly known reputation / credibility of their sources).
We use the value $\simparam{f} = 1/4$ for most of our simulations, but also show the impact of varying \simparam{f} on the created UCRs.

\item \textbf{\simparam{msp}} (\underline{m}ax \underline{s}hare \underline{p}robablility) models users' intrinsic sharing behavior: how likely users are to share news items they are exposed to.
For each simulated user $u$, we set $P_T(u)$ and $P_F(u)$ (see \cref{sec:detection-theory}) to a value chosen uniformly at random between $0$ and \simparam{msp}.
Note that \simparam{msp} is \emph{not} a system parameter of \systemname.
It models how users (which are external to \systemname) react to news items.
We do not know what \simparam{msp} is in reality.
We even expect it to be different for different news items, as, in reality, some items become viral (modeled by a high \simparam{msp}) and some do not (modeled by a low \simparam{msp}).
However, as we show later, regardless of what the real value of \simparam{msp} is,
\systemname\ effectively prevents fake items from going viral.
\end{itemize}

%% To present \systemname\ for a big and small value of \simparam{f}, we pick the $1/4$ and $1/64$, respectively.
%% Note that \simparam{f} refers to the fraction of fake items among the \emph{fact-checked} ones, and in general we can control which items are fact-checked and which are not.
%% If we try to pick popular items for fact-checking that are likely to be fake (e.g., based on some content-based machine learning algorithm, or items originating at sources known for spreading fake content), we can achieve a high fraction of fake items among those that we fact-check, making even \simparam{f} $=1/4$ a realistic value.

%% For \simparam{msp}, we pick $1/16$ and $1/64$\footnote{The expected probability of a user sharing an item is $\frac{\simparam{msp}}{2}$. (\cref{sec:simulation-setup})} as the respective big and small values.
%% Since we are concerned mostly about viral items, we choose the values for \simparam{msp} accordingly.
%% In our experiments we observe that \simparam{msp} $=1/16$ is the smallest value for which news items naturally become viral.
%% By ``viral'' we mean that an item naturally propagates to orders of magnitude more users than it was initially introduced to.
%%  %% for which the number of users exposed to it is orders of magnitude bigger than the number of users the item has been initially introduced to.
%% For \simparam{msp} $=1/32$ already, those numbers of users are of the same order of magnitude.
%% In order to illustrate how \systemname\ behaves for even smaller values, we also present experiments using \simparam{msp} $=1/64$.

%% COMMENT (M): mps depends on the tweet itself in reality, which is NOT
%% modeled by our system. However, tweets with low msp don't spread
%% naturally, and tweets with a high msp are efficiently handled by
%% \systemname.




%% Since we consider a limited subset of the tweets, our sample might not include some popular tweets.
%% This puts our estimation on the conservative side, as using more popular items would only improve the performance of our system.

%% We model the behavior of each user $u$ by $P_T(u)$ and $P_F(u)$, the respective probabilities that the user shares a true and a fake news item when exposed to it.
%% For each user, we initialize these share probabilities to random values uniformly distributed between 0 and \simparam{msp} (for maximal share probability).


\paragraph{\textbf{UCR Creation}}

To create UCRs, we propagate \simparam{r} items through the social graph.
We assign each of the \simparam{r} items a target share count.
The target share count corresponds to the number of retweets of a tweet in our dataset,
starting at the most popular one. % and using each tweet only once.
We randomly assign a (ground) truth value to each propagated item based on \simparam{f},
i.e., each item is fake with probability \simparam{f}.

The propagation itself proceeds by exposing a random user $u$ to the propagated item $X$ and having $u$ decide (probabilistically, based on $P_T(u)$ and $P_F(u)$) whether to share $X$ or not.
If $u$ shares $X$, we show $X$ to all $u$'s followers that have not yet seen it.
We repeat this process until one of the following conditions is fulfilled.
\begin{enumerate}
\item The target number of shares is reached.
  In this case we abort propagation immediately, possibly leaving some users without the possibility to decide whether to share $X$ or not.
\item At least 80\% of users have been exposed to $X$, at which point we consider the network saturated.
  This applies especially for small \simparam{msp} values, where the network becomes saturated without reaching the target share count.
  %% Such aborts have a negative impact on our results, since a fact-checked item affects fewer UCRs than it would in reality on a bigger social graph.
  %% In this sense, our simulations are thus a conservative approximation of the expected real-world behavior.
\end{enumerate}

%% An interesting detail about item propagation is the order in which we expose users to items.
%% For each item, we maintain a set of users that should be exposed to that item.
%% Whenever a user decides to share an item, we add all her followers to this set.
%% Users from this set are then exposed to the item in random order.
%% This is crucial, as with a more naive deterministic approach such as DFS traversal of the user graph, users would be exposed to items unevenly.
%% Especially for higher values of \simparam{msp} and lower target share counts, users appearing at the beginning of other users' lists of followers would be more likely to be exposed to an item than users at the end of the follower lists.
%% This would result in some users being exposed to many items (and thus have good UCRs) at the expense of other users.
%% Exposing items to users in random order solves this issue.

During item propagation, we keep track of how many true/fake items each user has seen/shared and update the UCRs accordingly.
%% Assuming all those items have been fact-checked, we update the UCRs accordingly.
%% We measure how various system parameters influence the quality of the obtained UCRs.
%% In particular,
%% \begin{enumerate}
%% \item How many fact-checked items users were exposed to,
%% \item How many UCRs have a relevant score, and
%% \item What are the values of these scores
%% \end{enumerate}



\paragraph{\textbf{Fake Item Detection}}

%% After having created the UCRs by simulating the propagation of fact-checked news items, we measure how effectively the obtained UCRs can be used to detect fake news.
In order to measure \systemname' fake news item detection capability,
we propagate $1000$ items through the social graph ($500$ fake and $500$ true).
We inject each item once, by making a random user $u$ share it.
The propagation happens as in the previous phase, with two important differences:
\begin{itemize}
\item We consider the item not fact-checked, and thus do not update $u$'s UCR.
  Instead, whenever $u$ is exposed to an item, we update that item's rating using the $u$'s UCR score.
  We use the share score if $u$ also shares the item, otherwise we use the view score (see \cref{sec:computing-fake-probability}).
\item We only propagate each item once, without re-inserting it when propagation dies off naturally.
\end{itemize}
When the probability of an item being fake reaches $p_0 = 0.999999$, we save the number of users exposed to it so far.
We continue spreading the item until the propagation stops naturally, to obtain the number of views that would occur in the absence of \systemname.

%% We consult $u$'s profile and include its view contribution (if $u$ did not share the item) or share contribution (if $u$ shared the item) in the computation of the item rating.
%% We measure:
%% \begin{enumerate}
%% \item The number of users that need to be exposed to an item before being reasonably certain that the item is fake.
%% This certainty is represented by the probability threshold $p_0 = 0.999999$.
%% If an item's probability of being fake exceeds $p_0$, we consider that item fake.
%% \item Total number of users exposed to the item.
%% \item Number of users exposed to the item if its propagation stops after being detected as fake.
%% \item Number of users that are prevented from being exposed to true items, if their propagation stops after being wrongly identified as fake.
%% \end{enumerate}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/reviewed-numContribsAbs}
\caption{The number of relevant UCR scores increases with both \simparam{r}, the number of fact-checked news items, and \simparam{f}, the fraction of these items that is fake.}
\label{fig:fact-checked-numContribsAbs}
%\vspace{-.3cm}
\end{figure}

\subsubsection{\textbf{Simulation Results}}\ \\

We now experimentally demonstrate \systemname' capability to effectively detect fake news items.
First we briefly describe how fact checking affects UCR creation and we discuss the choice of the used simulation parameters.
We then present our main result, namely the end-to-end impact of \systemname\ on the number of times users are exposed to fake news.

\paragraph{\textbf{Effectiveness of Fact-checkers}}

\systemname\ relies on fact-checked items to create UCRs.
Since a few most popular items usually reach a large number of users (see \cref{fig:tweet-popularity}),
our intuition is that checking only relatively few news items can result in obtaining sufficiently many useful UCRs.

While several aspects of UCRs influence \systemname' behavior,
due to space limitations we restrict ourselves to one representative metric of the overall quality of the UCRs present in the system:
the total number of UCRs with a useful UCR score.
We consider a UCR score useful if it is different from $1$,
i.e. when it makes a contribution to the rating of an item exposed to the corresponding user.

For this experiment, we choose $\simparam{msp} = 1/16$,
because (as we noticed empirically) this is a value where many items start naturally going viral.
By ``viral'' we mean that an item naturally propagates to orders of magnitude more users than it was initially introduced to.
%% For $\simparam{msp} = 1/32$ already, those numbers of users are of the same order of magnitude.

\Cref{fig:fact-checked-numContribsAbs} depicts how the number of relevant UCRs depends on \simparam{r},
the number of fact-checked items.
We see that fact-checking as few as 1024 news items has an impact on over 13M UCR scores,
which is one third of the whole user population.

The impact of \simparam{f} (the fraction of fake news items among the fact-checked ones) on UCRs is also shown in \cref{fig:fact-checked-numContribsAbs}.
While still assuming the majority of items being true, the higher the \simparam{f} parameter, the more useful UCRs we obtain.
This effect is due to the requirement of balanced UCRs described in \cref{sec:design}.

For the rest of our simulations, we use $\simparam{r} = 1024$ and $\simparam{f} = 1/4$,
as they provide good UCRs while still being a conservative choice.
FactCheck.org, for example, is one of many fact-checking initiatives that exist world-wide \cite{politifact,snopes,wpfactchecker,truthorfiction,fullfact}.
It checked several hundreds of popular stories only during the year 2017, the majority of which turned out to be false or misleading.

\paragraph{\textbf{Fake News Detection Capability}}
\label{sec:overall-effect}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/msp-viewCnt}
\caption{Fake news spreading with \systemname, as a function of \simparam{msp}. For low \simparam{msp}, news items do not become viral. For high \simparam{msp}, \systemname\ blocks the vast majority of fake news items.}
\label{fig:msp-viewCnt}

%\vspace{-.3cm}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/credulix-detail.pdf}
\caption{Fake news spreading with \systemname, as a function of \simparam{msp}, for different social graph sizes.}
\label{fig:msp-relative}
\end{figure}

The ultimate goal of \systemname\ is preventing fake news items from becoming viral on social media.
%% while allowing true news items to spread freely.
To this end, we measure the number of times a user is exposed to a fake news item in two scenarios:
%% We thus start by showing the overall effect of \systemname\ on fake news propagation.
%% To visualize this effect, we consider two scenarios:
\begin{enumerate}
\item Vanilla (natural) propagation of fake news items.
\item Propagation of fake items, where we stop propagating an item when \systemname\ labels it as fake.
\end{enumerate}
\Cref{fig:msp-viewCnt} presents results for items with varying rates of ``virality'', modeled by our \simparam{msp} simulation parameter.
It shows how many times a user has been exposed to a fake item, cumulatively over the $500$ fake items that we disseminate.
We can see that regardless of how viral the items would naturally become,
\systemname\ is able to timely detect the fake items before they spread to too many users.
\systemname\ restricts the number of views (cumulative over $500$ items) from hundreds of millions to tens or hundreds of thousands.%
\footnote{Analogously to a vaccine, \systemname\ needs \emph{some} fake news in order to function well,
as some users being exposed to fake news are crucial for obtaining meaningful UCRs.
Preventing the spreading of the vast majority of fake news might temporarily impair the effectiveness of \systemname, leading to an increased number of users being exposed to fake news.
This, in turn, reinforces \systemname' fake news detection capability.
We leave the study of such dynamic behavior to future work,
but we expect the fake news blocking rate to stabilize.
}

Especially nowadays, considering the increasing responsibility being attributed to social network providers as mediators of information,
it is crucial that true news items are not accidentally marked as fake.
We thus consider it very important to avoid false positives, i.e. true items being incorrectly labeled as fake.
None of these experiments encountered even a single false positive.

To have a closer look at the fake news detection rate,
we plot the percentage of fake items displayed with \systemname\ in \cref{fig:msp-relative}.
The more viral the items get (i.e. the higher the \simparam{msp} value), the more effective \systemname\ becomes at fake item detection.
Intuitively, the more items users share, the more precisely we are able to estimate their sharing behavior.

While not visible in the plot, it is worth noting that not only the relative amount of viewed fake items decreases, but also the \emph{absolute} one.
(One could think that the relative decrease for \systemname\ is only due to an absolute increase for Baseline.)
Interestingly, with increasing tendency of items to go viral (i.e. increasing \simparam{msp}),
even the \emph{absolute} number of displayed fake items decreases.
This effect is due to a higher \simparam{msp} value ensuring more spreading of (both true and fake) news items in our UCR creation phase (see \cref{sec:simulation-methodology}).
This in turn produces better UCRs, increasing \systemname' effectiveness.

\Cref{fig:msp-relative} also conveys the effect of the size of the social graph on the performance of \systemname.
On a smaller graph of 1M users generated with the SNAP generator \cite{snapnets},
\systemname\ achieves a lower fake item detection rate.
This is because the impact of fact-checked items is smaller on a small graph, leading to fewer users with relevant UCR scores.
%% , on which the effectiveness of \systemname\ relies.
This result suggests that on a real social graph, which is even larger than the one we use, \systemname\ would perform even better than in our simulation.

%% As we will explain in detail later, the parameter most influential to \systemname' behavior is \simparam{msp}.
%% The higher \simparam{msp}, the more quickly and accurately we are able to detect fake news items.

%% We show that even so, regardless of \simparam{msp}, fake news items never become viral when \systemname\ is in place.
%% \cref{fig:msp-viewCnt} depicts how the number of users exposed to a fake item depends on \simparam{msp}, for both above-mentioned scenarios.
%% The "Vanilla" lines coincide, because without \systemname, fake item propagation does not depend on \simparam{r} or \simparam{f}.
%% Note that for low values of \simparam{msp}, an item naturally does not spread enough to become viral.
%% As \simparam{msp} grows, our system becomes more and more effective at detecting fake news items, preventing them from spreading at an early stage of propagation.

%% We do not include plots for true news items as those also coincide with the top 3 "Vanilla" lines in both scenarios (both with and without \systemname).
%% This means that the \systemname 's impact on true news items is negligible.


% \cref{fig:msp-viewCnt} contains 6 lines, 3 of which coincide.
% The 3 coinciding lines at the top represent the the number of times a fake item is shown to a user, without the use of \systemname\ (Vanilla)
% The 3 lines at the bottom represent the number of times a fake item is shown to a user with \systemname, for 3 different parametrizations.
% It is clear that from the image that \systemname\ is able to prevent the propagation of fake items, while leaving true items to propagate freely.

%% In the rest of \cref{sec:effectiveness-of-detection}, we present other interesting measurements that help explain the behavior of \systemname.

% So far we studied the effectiveness of our solutions to sub-problems of fake news elimination.
% We now present the end-to-end effect of our system on the spreading of fake news items through a social network.
% We are interested in how many users are actually exposed to fake news as compared to the number of users who would have been affected if our system was not in place.

% As becomes evident from the previously mentioned results, the most crucial parameter determining the effectiveness of our system is \simparam{msp}.
% In reality, the probability of an item being shared by a user is not static, but depends also on the item itself, which is not captured by our simulations.
% This is what, in reality, makes the difference between a viral news item and one that does not become viral.

% The crucial role of the $msp$ parameter lies in ensuring good user profiles, as can be seen in Figure ??.
% This is natural, as a higher $msp$ during the propagation of fact-checked news items ensures a higher number of users being exposed to these items.
% This not only helps increase the user profile scores more, but, most crucially, increases the chance that a profile with high score will also have a strong contribution.

% In our simulations, we use the same static value for $msp$ throughout both profile creation and fake item detection.
% From this point of view, Figure ?? is a conservative approximation of reality, as it is the most viral items that are being fact-checked, corresponding to a rather high $msp$ value.

%% First, we study the effect of fact-checking popular news items on UCRs.
%% Since a few most popular items usually reach a large number of users (see \cref{fig:tweet-popularity}), our intuition is that checking only relatively few news items can create ``good'' UCRs.
%% % that are sufficiently good for effective fake news detection.
%% The general quality of a UCR could be expressed in terms of the number of fact-checked items that user has been exposed to.
%% However, due to the way we compute UCRs in practice (see \cref{sec:design-principles}), the number of fact-checked items relevant for a UCR is only $\min(v_T, v_F)$.
%% \cref{fig:fact-checked-score} shows the average value of $\min(v_T, v_F)$ over all users as a function of \simparam{r}, i.e., the number of fact-checked items.

% \begin{figure}
% \centering
% \includegraphics[width=\columnwidth]{figures/reviewed-score}
% \caption{Average value of $\min(v_T, v_F)$ over all users, as a function of \simparam{r}, \simparam{f}, and \simparam{msp}. It increases with \simparam{r} and \simparam{f}, but is unaffected by \simparam{msp}.}
% \label{fig:fact-checked-score}
% %\vspace{-.3cm}
% \end{figure}

%% Note that the values increase not only with the number of fact-checked items, but also with \simparam{f}, the overall fraction of fake news in the system.
%% This is due to the fact that having a more even distribution of true and fake fact-checked news items, $\min(v_T, v_F)$ increases while $(v_T + v_F)$ remains the same.
%% While the value of $\min(v_T, v_F)$ gives us an insight about the relevance of $r$ and $f$, maximizing it is necessary, but not sufficient for efficient fake news detection.
%% A user $U$ might be exposed to many true and fake fact-checked items, but if $U$ does not share any of these items, $U$'s UCR score is still $1$ and thus not useful for fake news detection.
%% The same goes for a user sharing all items she is exposed to.

%% The most important property of a UCR is its score (see \cref{sec:design-principles}).
%% Recall that an item rating is computed as a product of UCR scores for all users exposed to that item.
%% Thus, the more UCRs have a score different from 1, the more effectively fake news items can be detected.

%% \cref{fig:fact-checked-numContribsAbs} shows the number of UCR scores different from $1$, depending on the number of fact-checked items \simparam{r}.
%% This time, the results depend not only on \simparam{f}, but on \simparam{msp} as well.
%% For the reasons explained above, the more likely a user is to share an item, the more likely it is that her UCR will have a relevant score.

% \begin{figure}
% \centering
% \includegraphics[width=\columnwidth]{figures/reviewed-contribFact}
% \caption{The UCR score values also increase with all of \simparam{r}, \simparam{f}, and \simparam{msp}.}
% \label{fig:fact-checked-contribFact}
% %\vspace{-.3cm}
% \end{figure}

%% \begin{figure}
%% \centering
%% \includegraphics[width=\columnwidth]{figures/viewCnt-detectionRate}
%% \caption{Effectiveness of fake news item detection for \simparam{r}~$=1024$. We display the CDF of fake news items detected, depending the number of users exposed to each item. The horizontal axis uses a logarithmic scale.}
%% \label{fig:viewCnt-detectionRate}
%% %\vspace{-.3cm}
%% \end{figure}

%% It is not only important how many UCRs with relevant scores there are, but what values these scores have.
%% A score close to $1$ is not as useful as a score with a bigger difference to $1$.
%% The further the UCR scores are from $1$, the fewer of them need to be considered to reach the same level of confidence in an item being true or fake.
%% In \cref{fig:fact-checked-contribFact}, we plot the average factor by which a UCR score differs from $1$.
%% As expected, the bigger \simparam{msp}, \simparam{f} and \simparam{r}, the better the score.

%% \subsubsection{Fake News Detection}

%% %% Previously we only studied how various parameters affect the quality of user profiles.
%% In this experiment, we show how effectively \systemname\ detects fake news items.
%% We are interested in the number of views necessary for fake item detection.
%% I.e., how many users have to be exposed to a fake news item in order for the system to detect it as fake.
%% Assuming that the system would block the propagation of a news item detected to be fake, this metric directly expresses how effectively \systemname\ can be used to prevent exposing users to fake news.

%% \cref{fig:viewCnt-detectionRate} plots the fractions of detected fake items relative to the number of users that have been exposed to those items.
%% We see that for \simparam{f} $=1/4$ and \simparam{msp} $=1/16$, all fake items are detected after being viewed by $8196$ users, while most fake items -- 93.6\% and 99.8\% -- are already revealed after being seen by $2048$ and $4096$ users respectively.
%% For the small \simparam{msp} $=1/64$, it might take tens of thousands of user views until an item is detected as fake.
%% However, in the presented experiments, the propagation of these items often died off naturally even before sufficient number of UCRs could be considered (see also \cref{sec:overall-effect}).
%% None of the items reached $2^{17} \approx 130$k users.


%% The point on the trade-off between false positives and false negatives can be tuned using the threshold that needs to be exceeded by a item's probability of being fake in order for the item to be considered fake.
%% We tend to choose a number very close to 1 for this threshold in order to avoid false positives.
%% For 3 out of the 4 experiments in \cref{fig:viewCnt-detectionRate}, we did not observe any false positives.
%% In the experiment with the most pessimistic parametrization of \simparam{f} $=1/64$ and \simparam{msp} $=1/64$, the rate of false positives was less than $1.8\%$.


\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/latency-experiments-figure.pdf}
\caption{Throughput and latency cost of \systemname.}
\vspace{-.3cm}
\label{fig:system-eval-fig}
\end{figure*}

\subsection{\systemname\ Overhead}
In this section we evaluate \systemname' impact on user operation (viewing and sharing) throughput and latency when plugged into a social network.

\subsubsection{\textbf{Experimental Setup}}\ \\

Here we evaluate an implementation of \systemname\ as a stand-alone Java plugin.
We implement a Twitter clone\footnote{Where the share and view operations are identical to \cref{fig:tweet-operation,fig:timeline-operation}}.
From this point forward, we refer to our Twitter clone as the \emph{Baseline}
and to the system with \systemname\ plugged in as \systemname.
For the data store of the Baseline we use Twissandra's data store\cite{twissandra},
running Cassandra version 2.2.9\cite{cassandra}.

We conduct our evaluation on a 48-core machine,
with four 12-core Intel Xeon E7-4830 v3 processors operating at 2.1 GHz,
512 GB of RAM and a 400 GB SSD Samsung 843T, running Ubuntu 16.04.
We run our experiments on a real-world Twitter graph of over 41M users \cite{Kwak10www}, as in \cref{sec:effectiveness-of-detection}.
Each experiment consists of 16 worker threads concurrently performing operations on the social network (sharing items or viewing news feeds).
Each operation is chosen at random, according to the given workload probability distribution.
Each user is chosen uniformly at random from the all the users in the social network graph.

We run two types of workloads.
The first has 90\% view operations and 10\% share operations (already a high percentage of share operations for a realistic social network). The second is a view-only workload. We run each experiment 5 times and we take the average of the results. For the sake of fairness, in each experiment, both \systemname\ and the Baseline use the same execution trace, which was generated a priori. An execution trace is a list of user IDs and operations (e.g., user1:share, user2:view etc.). For all our experiments we consider a user to be influential if they are among the 5\% most followed users.

\subsubsection{\textbf{Experimental Results}}\ \\

\Cref{fig:system-eval-fig} conveys the latencies of user operations, along with the throughput of \systemname\ relative to the Baseline.
The mixed workload is shown on the left side, and the view-only workload is shown on the right side of the figure.

The additional overhead in terms of throughput and latency incurred by \systemname\ is low.
The throughput penalty caused by \systemname\ is between 3\% (in the view-only workload) and 9\% (in the mixed workload).
The impact on throughput is predominantly caused by \systemname' background tasks, as detailed in \cref{sec:design}. 

Latency increases by at most 3\%, at the $90^{th}$ percentile.
The low overhead in latency is due to \systemname\ keeping its computation  outside the critical path.
Standard deviation of latencies is high both for the Baseline and for \systemname, for both post and check operations.
The high variation in latency is caused by the intrinsic differences between the users;
for instance, post operations of a user with more followers need to propagate to more users than posts of users with few or no followers.

The high $99^{th}$ percentile latency for both systems results from Twissandra (our Baseline) being implemented in Java,
a language that is (in)famous for its garbage collection breaks.
Certain operations, during which garbage collection is performed by the JVM, thus experience very high latencies.
This effect is not inherent to the system itself,
but is merely an artifact of its Java implementation and can be avoided by using a language with explicit memory management.
The impact of garbage collection is stronger with \systemname\ than with Baseline,
as \systemname\ creates more short-lived objects in memory to orchestrate its background tasks.
In addition to the intrinsic differences between users discussed above,
garbage collection also significantly contributes to the high standard deviation observed in all latencies.

%% For identical traces run by the Baseline and by \systemname, the latency standard deviation is higher in \systemname.
%% This is due to the fact that, while a significant fraction of the posts are not tracked (thus incurring no overhead),
%% for the posts that are tracked, \systemname\ does perform additional operations.
%% Even if the bulk of the work is performed in the background,
%% there is still overhead associated to starting the background task,
%% causing an increase in latency. 

%% We also notice a significant difference in the 99th percentile latency (18\% in the mixed workload and 40\% in the view-only workload) between \systemname\ and the Baseline.
%% This is due to the fact that \systemname\ is generating background-task objects in order to track items on the read path.
%% These tasks are small and short lived, thus adding extra work for the garbage collector compared to the Baseline.
%% Note that this limitation of the implementation can be avoided in a language providing manual memory management,
%% for example by using a pre-allocated memory pool for such tasks and recycling the memory. 


==> sections/theory-alex.tex <==
\section{Theoretical Foundations}
\label{sec:theory}
In this section we present the theoretical foundations underlying \systemname.
We give an intuition of our result, followed by its formalization as a theorem.
We also show how to restate the very same problem in a way that allows efficient computation of news item credibility.

\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{figures/fake-news-intro-schema.pdf}
\vspace{-.7cm}
\caption{News item falsehood probability computation.} 
\label{fig:schemebayes}
\end{center}
\vspace{-.5cm}
\end{figure}

\subsection{Intuition}
The context is a social network where users can post news items, such as links to newspapers or blog articles.
Users exposed to these news items can in turn share them with other users (Twitter followers, Facebook friends etc.). The social network has a fact-checking team whose role is to determine whether certain news items are fake (according to some definition of fake)\footnote{Our truth and falsehood criteria here are as good as the fact-checking team.}. The news items that the fact-checking team needs to check is very low compared to the total number of items in the social network.

\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{figures/classificationexample.pdf}
\vspace{-.7cm}
\caption{Users reacting to new item $X$.} 
\vspace{-.5cm}
\label{fig:toyex}
\end{center}
\end{figure}

\subsubsection{The Main Steps}
\label{sec:main-steps} 
Our approach goes through the following three main steps: 
\begin{enumerate}
\item	The fact-checking team reviews few news items (ideally those that have been the most viral ones in the past). This is considered the ground truth in our context.
\item   \systemname\ creates a probabilistic model of each user's sharing behavior based on their reactions (share / not share) to the fact-checked items in Step (1).
  This captures the likelihood of a user to share true (resp. fake) news items.
\item	For a new, unchecked news item $X$, we use the behavior models generated in Step (2) to determine the probability that $X$ is fake, based on who viewed and shared $X$.
\end{enumerate}


% We compute the probability of a news item $X$ being fake based on
% (1) the estimated overall fraction of fake items in the social network and
% (2) the modeled sharing behavior of users exposed to $X$.



%% two major components: one stemming from the ground truth, shown on the right side of the figure, and a dynamic component, determined by the users who were exposed to $X$ in real time, shown on the left side of the figure.

%% (M) The thing with the two components is slightly confusing to me and seems unnecessary.

%% The ground truth allows us to estimate the global fraction of fake news in the social network (or a lower bound) --- an important parameter for \systemname. Moreover, the ground truth allows us to model the user sharing behavior, which we store in User Credulity Records, or UCRs. We describe UCRs in detail in the following subsection. 

%% (M) Maybe details that don't need to go here yet? Also, let's discuss how to explaint the ``important parameter''.

%% After the UCR creation, we then observe how users react to items that have not been fact-checked.
A high-level view of our technique is depicted in \cref{fig:schemebayes}.
We use a Bayesian approach. For example, if an item is mostly shared by users with high estimated probabilities of sharing fake items, while users with high estimated probabilities of sharing true items rarely share it, we consider the item likely to be fake (\cref{fig:toyex}).

\subsubsection{Preventing the Spread of Fake News} 
Once we estimate the probability of a news item $X$ being fake, preventing its spread becomes easy. Let $p_0$ be any cutoff probability threshold. Each time a user views or shares $X$, we compute $p$, the probability of $X$ being fake, which we detail below. If $p \geq p_0$ (i.e., $X$ has a probability at least $p_0$ to be fake),
\systemname\ stops showing $X$ in the news feed of users, preventing $X$ from spreading and becoming viral.

\subsection{Fake News Detection}
\label{sec:detection-theory}
%% \vspace{-2mm}
\subsubsection{User Behavior} 
We model the behavior of a user $u$ using the two following probabilities:
%% \vspace{-1mm}
\begin{itemize}
\item $P_T(u)$: probability that $u$ shares a news item if it is true.
\item $P_F(u)$: probability that $u$ shares a news item if it is fake.
\end{itemize}

The probabilities $P_T(u)$ and $P_F(u)$ are assumed to be independent between users. In practice, this is the case if the decision to share a news item $X$ is mainly determined by $X$ itself. 
% One could object that some users may be subject to a certain level of social influence. For instance, if $X$ has already been shared by many contacts of $u$, it could make $u$ more (or less) likely to share $X$ (depending on how $u$ responds to social influence). However, the inputs of our model do not give information on these possible effects. Besides, the probabilities $P_T(u)$ and $P_F(u)$ already encompass the average effect of social influence on $u$. Finally, the users involved in the formula do not necessarily represent a large fraction of $u$'s contacts. Thus, it is reasonable to model these probabilities as independent.

We obtain estimates of $P_T(u)$ and $P_F(u)$ for each user based on the user's behavior (share / not share) with respect to fact-checked items. For any given user $u$, let $v_T(u)$ (resp. $s_T(u)$) denote the number of fact-checked true news items \emph{viewed} (resp. \emph{shared}) by $u$, and $v_F(u)$ (resp. $s_F(u)$) the number of fact-checked fake news items \emph{viewed} (resp. \emph{shared}) by $u$.
We call the tuple $(v_T(u), s_T(u), v_F(u), s_F(u))$ the \emph{User Credulity Record} (UCR) of $u$.

User behavior has been modeled similarly in prior work, for instance, in Curb \cite{Curb}. In Curb, users exposed to a news item decide probabilistically whether to share it, potentially exposing all their followers to it. Curb relies on very similar metrics, namely the numbers of viewed and shared items for each user, and the probabilities that users would share true or false news items.


%% \begin{table}
%% \centering
%% \bgroup
%% \def\arraystretch{1.5}%  1 is the default, change whatever you need
%% \begin{tabular}{|r|l|}
%% \hline
%% $v_T(u)$ & Number of fact-checked \emph{true} items \emph{viewed} by $u$ \\
%% \hline
%% $s_T(u)$ & Number of fact-checked \emph{true} items \emph{shared} by $u$ \\
%% \hline
%% $v_F(u)$ & Number of fact-checked \emph{false} items \emph{viewed} by $u$ \\
%% \hline
%% $s_F(u)$ & Number of fact-checked \emph{false} items \emph{shared} by $u$ \\
%% \hline
%% \end{tabular}
%% \egroup
%% \caption{User Credulity Record (UCR)}
%% \label{tab:ucr}
%% \end{table}
For any given user $u$, we define the following functions, based on the UCR:

\begin{itemize}


\item $\beta_1(u) = ( s_T(u)+1 ) / ( v_T(u)+2 )$
\item $\beta_2(u) = ( s_F(u)+1 ) / ( v_F(u)+2 )$
\item $\beta_3(u) = ( v_T(u) - s_T(u) +1 ) / ( v_T(u)+2 )$
\item $\beta_4(u) = ( v_F(u) - s_F(u)+1 ) / ( v_F(u)+2 )$

\end{itemize}

According to Laplace's Rule of Succession \cite{Zabell1989}, we have $P_T(u) = \beta_1(u) $ and 
$P_F(u) = \beta_2(u) $.


\subsubsection{Probability of a News Item Being Fake}
\label{sec:fake-detection}
At the heart of \systemname\ lies a formula to compute the likelihood of a new (not fact-checked) news item $X$ to be fake. Let $V$ and $S$ be any two sets of users that have \emph{viewed} and \emph{shared} $X$, respectively. The probability that $X$ is fake, $p(V,S)$ is computed as:
%% \vspace{-.2cm}

\begin{equation}
\label{eq:formula}
\boxed{p(V,S) = g\pi_F(V,S)/(g\pi_F(V,S) + (1-g)\pi_T(V,S))}
\end{equation}

\noindent{Where:}
\begin{itemize}
\item $\pi_T(V,S) = \prod_{u \in S} \beta_1(u) \prod_{u \in V - S}  \beta_3(u)$
\item $\pi_F(V,S) = \prod_{u \in S} \beta_2(u) \prod_{u \in V - S} \beta_4(u)$, and
\item $g$ is the estimated \emph{global fraction} of fake news items in the social network, with $g \in$ $(0,1)$.
\end{itemize}

$g$ can be estimated by fact-checking a set of news items picked uniformly at random from the whole social network.
Let $g^*$ be the real fraction of fake news items in the social network. We distinguish two cases: $g^*$ is known, and $g^*$ is unknown. If $g^*$ is known, we have the following theorem.

\begin{theorem}
\label{thmprob}
Let $g = g^*$.
A news item \emph{viewed} by a set of users $V$ and \emph{shared} by a set of users $S$ is fake with probability $p(V,S)$.
\end{theorem}

\begin{proof} 

Consider a news item $X$ that has not been fact-checked. Consider the following events:
\begin{itemize}
\item[$E$]: $X$ viewed by a set of users $V$ and shared by a set of users $S$.
\item[$F$]: $X$ is fake.
\item[$T$]: $X$ is true.
\end{itemize}

Our goal is to evaluate $P(F|E)$: the probability that $X$ is fake knowing $E$.

\begin{itemize}

\item If $X$ is true, the probability of $E$ is $P(E|T) =$ \\$\prod_{u \in S} P_T(u) \prod_{u \in V - S} (1 - P_T(u)) = \pi_T(V,S)$.

\item If $X$ is fake, the probability of $E$ is
$P(E|F) =$
\\$\prod_{u \in S} P_F(u) \prod_{u \in V - S} (1 - P_F(u)) = \pi_F(V,S)$.

\end{itemize}


The probability that $X$ is fake (independently of $E$) is $P(F) = g^*$,
and the probability that $X$ is true (independently of $E$) is $P(T) = 1 - g^*$.

Thus, we can determine the probability that $E$ is true:
$P(E) = P(E|T)P(T) + P(E|F)P(F) = (1-g^*)\pi_T(V,S) + g^*\pi_F(V,S)$.

$P(F|E) = P(E|F)P(F)/P(E)$ according to Bayes' Theorem \cite{Koch1990}.
Then, $P(F|E) = g^*\pi_F(V,S)/(g^*\pi_F(V,S) + (1-g^*)\pi_T(V,S)) = p(V,S)$. Thus, the result.\end{proof}




If $g^*$ is unknown, we assume that $g$ is a lower bound of $g^*$. We get in this case the following theorem.

\begin{theorem}
\label{thmprob2}
For $g \leq g^*$, a news item \emph{viewed} by a set of users $V$ and \emph{shared} by a set of users $S$ is fake with probability \emph{at least} $p(V,S)$.
\end{theorem}

\begin{proof}

First, note that $\pi_T(V,S)$ and $\pi_F(V,S)$ are strictly positive by definition.
Thus, the ratio $\pi_T(V,S)/\pi_F(V,S)$ is always strictly positive.

$\forall x \in (0,1)$,
let $g(x) = x \pi_F(V,S) / ( x \pi_F(V,S) $ + $(1-x) \pi_T(V,S) )$.

Then, $p(V,S) = h(g)$, and 
according to Theorem~\ref{thmprob}, the news item is fake with probability $h(g^*)$. 

Written differently, $g(x) = 1 / (1 + k(x))$, with $k(x) = (1/x - 1) \pi_T(V,S) / \pi_F(V,S)$.

As $g \leq g^*$, $1/g \geq 1/g^*$, $1 + k(g) \geq 1 + k(g^*)$
and $h(g) \leq h(g^*)$. Thus, the result.\end{proof}

\subsection{Efficiently computing news item credibility}
\label{sec:computing-fake-probability}

%% The effectiveness of \systemname\ relies on the fact that the probability of a news item being fake can be computed efficiently.
\systemname' measure of credibility of a news item $X$ is the probability $p(V,S)$ that $X$ is fake.
An obvious way to compute this probability is to recalculate $p(V,S)$ using \cref{eq:formula} each time $X$ is viewed or shared by a user.
Doing so, however, would be expensive in terms of computation\footnote{A number of operations larger than the number of users that have viewed $X$ so far.}.
Below, we show an efficient method for computing news item credibility.
We first describe the computation of UCRs,
and then present our fast, incremental approach for computing news item credibility using \emph{item ratings} and \emph{UCR scores}.
%% We adopt a much faster, \emph{incremental} technique to check if $p(V,S) \geq p_0$ (the cutoff probability threshold).
%% To this end, we introduce the notions of \emph{item rating} and \emph{UCR score}.
\subsubsection{Computing User Credulity Records (UCRs)}
%% For each user, we store the \emph{User Credulity Record (UCR)}, as defined in \cref{sec:theory}.
Recall that the four values $(v_T(u)$, $s_T(u),$ $v_F(u),$ $s_F(u))$ constituting a UCR only concern \emph{fact-checked} news items.
We thus update the UCR of user $u$ in the following two scenarios.
% \begin{itemize}
% \item $v_T$: the number of true viewed news items
% \item $s_T$: the number of true shared news items
% \item $v_F$: the number of fake viewed news items
% \item $s_F$:  the number of fake shared news items
% \end{itemize}
\begin{enumerate}
\item When $u$ views or shares a news item that has been fact-checked (i.e., is known to be true or fake).
\item Upon fact-checking a news item that $u$ had been exposed to.
%% we iterate through all the users who have been exposed to $T$ and increment the corresponding UCR values, based on whether they shared $T$ or not, as well as based on the truth value of $T$.
\end{enumerate}

In general, the more fact-checked news items a user $u$ has seen and shared, the more \emph{meaningful} $u$'s UCR. Users who have not been exposed to any fact-checked items cannot contribute to \systemname. 
%On the other hand, if $U$ is  exposed to many fact-checked items and mostly shares the true ones among them, while sharing none of the fake ones, \systemname\ infers that $U$ is more likely to share true items.

% For \systemname\ to work best, it is necessary that UCRs are \emph{balanced}.
% This means that there are as many true viewed items as there are fake ones (i.e., $v_T(u) = v_F(u)$).
% %% This is difficult to achieve in practice, since the items which users are exposed to is out of our control.
% %% Furthermore, the overall ratio between true and fake news items on the network can be inherently unbalanced.
% In order to achieve balanced UCRs for the purposes of our computation, we consider $\min(v_T, v_F)$ for both $v_T$ and $v_F$.\\
% We then restrict $s_T$ and $s_F$ to be the numbers of shared news items among the most recently seen $v_T$ true and $v_F$ fake fact-checked items, respectively. The reason for this choice is the following. When $v_T(u)$ and $v_F(u)$ are small, $P_T(u)$ and $P_F(u)$ tend to be biased towards the \emph{a priori} probability (based on the fraction of fake news). When both are ``equally biased'' towards this value, the ratio is stable. However, when one is biased and the other is not, the ratio becomes unstable. This, of course, does not prevent the probabilities to converge to the exact value for an arbitrarily large number of data points. However, in practice, for a limited number of data points, this phenomenon significantly decreases the quality of our estimations. Thus, we choose to keep $v_T(u)$ and $v_F(u)$ equal. Given that these two quantities are equal, it is beneficial for \systemname\ to have a larger amount of fake items in the ground truth than the global fraction of fake news in the social media platform. This is obtained by biasing the sampling process using \simparam{f}, as explained in the previous section.


\subsubsection{Item Rating}
In addition to $p(V,S)$, we introduce another measure of how confident \systemname\ is about $X$ being fake: the \emph{item rating} $\alpha(V,S)$, whose role is equivalent to that of $p(V,S)$.
We define it as $\alpha(V,S) = \pi_T(V,S)/\pi_F(V,S)$, $V$ and $S$ being the sets of users that viewed and shared $X$, respectively.
If we also define $\alpha_0 = (1/p_0 - 1) / (1/g - 1)$ as the rating threshold corresponding to the probability threshold $p_0$,
then, $p(V,S) \geq p_0$ is equivalent to $\alpha(V,S) \leq \alpha_0$\footnote{We have $p(V,S) = g \pi_{F}(V,S) / ( g \pi_{F}(V,S) + (1-g) \pi_{T}(V,S) )
= g / ( g  + (1-g) (\pi_{T}(V,S) / \pi_{F}(V,S) ) ) =  g / ( g  + (1-g) \alpha(V,S) )$.
We have $p(V,S) \geq p_{0}$ if and only if $g/p(V,S) \leq g/p_0$, that is:
$g + (1-g) \alpha (V,S) \leq g/p_{0}$,
which is equivalent to
$\alpha (V,S) \leq (1/p_0 - 1)/(1/g - 1)$,
that is:
$\alpha (V,S) \leq \alpha_0$.}.
When the item $X$ with $\alpha(V,S) \leq \alpha_0$ is about to be displayed in a user's news feed, \systemname\ suppresses $X$.
Note that $\alpha_0$ can be a fixed constant used throughout the system, but may also be part of the account settings of each user,
giving users the ability to control how ``confident'' the system needs to be about the falsehood of an item before suppressing it.

\subsubsection{UCR Score}
According to the definition of $\pi_T(V,S)$ and $\pi_F(V,S)$ in \cref{sec:detection-theory},
each time $X$ is viewed (resp. shared) by a new user $u$,
we can update the $X$'s rating $\alpha(V,S)$ by multiplying it by $\gamma_v(u) = \beta_1(u)/\beta_2(u)$ (resp. $\gamma_s(u) = \beta_3(u)/\beta_4(u)$).
We call $\gamma_v(u)$ and $\gamma_s(u)$ respectively the \emph{view score} and \emph{share score} of $u$'s UCR, as their value only depends on $u$'s UCR (see \cref{sec:detection-theory} for definition of UCR).
Consequently, when a user views or shares $X$, we only need to access a single UCR in order to update the rating of $X$. This is what allows \systemname\ to update news item credibility fast, without recomputing eq. (1) each time the item is seen by a user.

In what follows, we refer to $\gamma_v(u)$ and $\gamma_s(u)$ as $u$'s \emph{UCR score}.
% Intuitively, the UCR score captures the influence of $u$'s UCR on the rating of items that $u$ views and shares.
The more a UCR score differs from $1$, the stronger its influence on an item rating (which is computed as a product of UCR scores).
We consider a UCR score to be \emph{useful} if it is different from $1$.
% This is what we refer to as a \emph{high} UCR score.


%% \noindent\textbf{UCR score.} Recall that we estimate the truth value of a news item $T$ based on the UCRs of users who have seen $T$ and whether those users shared $T$ or not. The \emph{influence} of a UCR on T's rating is captured by what we call its \emph{score}. More precisely, $T$'s rating is a product of UCR scores across all users that were exposed to $T$.
%% We distinguish two kinds of UCR scores. Only one of the two scores is used at a time for a given item.
%% \begin{enumerate}
%% \item \emph{View score}. The UCR score of a user who viewed $T$, but did \emph{not} share it.
%% \item\emph{Share score}. The UCR score of a user who viewed and also shared $T$.
%% \end{enumerate}

%% \noindent\textbf{News items.} \systemname\ augments news items with an
%% \emph{item rating}. The rating is a measure of how confident
%% \systemname\ is that the news item is true or fake.  Whenever an item
%% is displayed to a user $U$ on the social network, we update the item
%% rating by $U$'s \emph{UCR view score}. When $U$ shares a news item, we
%% update the item rating by $U$'s \emph{share score}. Whenever a news
%% item is about to be displayed in $U$'s news feed, we suppress the item
%% if its rating exceeds a certain predefined threshold. Note that this
%% threshold may be a fixed constant used across the whole system, but
%% may also be part of the account settings for each user, giving users
%% the ability to control how ``confident'' the system needs to be about
%% the falsehood of an item before suppressing it.

%% \subsubsection{Fake Items Fraction}
%% \begin{figure}
%% \begin{center}
%% \includegraphics[width=\columnwidth]{figures/fact-checkB.pdf}
%% \caption{Global fake news fraction \emph{g} and the fraction of fake items in the ground truth \simparam{f}.} 
%% \label{fig:fact-checking}
%% \end{center}
%% \vspace{-3mm}
%% \end{figure}

%% \systemname\ makes use of \emph{two different} fake news fractions: the fraction of fake items \emph{in the ground truth}, which we call \simparam{f}, and the \emph{global fraction of fake items in the social media platform}, denoted by \emph{g} (in eq. (1)).
%% %\cref{fig:fact-checking} illustrates the differences between these two quantities and the way in which they are obtained. 

%% The global fraction of fake items in the social media platform \emph{g} is \emph{not} a parameter of \systemname. We, however, need an estimate of \emph{g} in order to compute the likelihood of items being fake. We estimate \emph{g} by uniform sampling and fact-checking of news items.%, as depicted in \cref{fig:fact-checking}.

%% On the other hand, \simparam{f} is a parameter of \systemname\ that we set and then use for biased sampling of items which are fact-checked. These are then used to model users' sharing behavior. We show the impact of different values of \simparam{f} in \cref{sec:evaluation}. The fact-checked items necessary to achieve \simparam{f} are picked as much as possible from the most popular ones, to ensure they are seen by many users in the network. Moreover, to achieve the desired fact-checked fake news fraction (i.e., \simparam{f}), it is possible to have the fact-checked items set include items from sources that are biased towards fact-checking fake items. FactCheck.org, for example, is one of many fact-checking initiatives that exist world-wide \cite{politifact,snopes,wpfactchecker,truthorfiction,fullfact}.
%% It checked several hundreds of popular stories only during the year 2017, the majority of which turned out to be false or misleading.





%% The value $\alpha(V,S)$ can also be computed in a distributed way.
%% Let $(V_i,\dots,V_n)$ be $n$ disjoint sets of users that have viewed the news item.
%% For instance, each $i$ can correspond to a local server of the social network.
%% For $i \in \{1,\dots,n\}$,
%% let $S_i \subseteq V_i$ be the corresponding set of users that have shared the news item.
%% Each local server $i$ computes $\alpha(V_i,S_i)$.
%% Then, $\alpha(V,S) = \prod_{i \in \{1,\dots,n\}} \alpha(V_i,S_i)$.

%% (M) Instead of the previous paragraph: As $\alpha(V_i,S_i)$ is a product of the values $\gamma_v$ or $\gamma_s$ of different users


